On Measuring Excess Capacity in Neural Networks

We study the excess capacity of deep networks in the context of supervised classification. That is, given a capacity measure of the underlying hypothesis class - in our case, empirical Rademacher complexity - to what extent can we (a priori) constrain this class while retaining an empirical error on a par with the unconstrained regime? To assess excess capacity in modern architectures (such as residual networks), we extend and unify prior Rademacher complexity bounds to accommodate function composition and addition, as well as the structure of convolutions. The capacity-driving terms in our bounds are the Lipschitz constants of the layers and an (2, 1) group norm distance to the initializations of the convolution weights. Experiments on benchmark datasets of varying task difficulty indicate that (1) there is a substantial amount of excess capacity per task, and (2) capacity can be kept at a surprisingly similar level across tasks. Overall, this suggests a notion of compressibility with respect to weight norms, complementary to classic compression via weight pruning. Source code is available at https://github.com/rkwitt/excess_capacity.

==> figs/adv_examples/attacks.tex <==
\newcommand{\plotattack}[5]{
    \begin{scope}[xshift=#2, yshift=#3]
    \begin{axis}[
        width = .525\textwidth,
        height = 4cm,
        legend pos = south west,
        legend cell align = left,
        legend style = {font=\tiny},
        %
        title = {\textbf{#1}},
        title style = {font=\tiny, yshift=-.5em},
        %
        xlabel = {\ifthenelse{\equal{#5}{1}}{Attack strength}{}},
        ylabel = {\ifthenelse{\equal{#4}{1}}{Fraction of \textbf{correctly} \\classified images}{}},
        xlabel style = {font=\tiny, yshift=.5em},
        ylabel style = {align=center, font=\tiny, yshift=-3pt},
        tick label style = {font=\tiny},
        legend style = {font=\tiny, draw = none},
        %
        enlargelimits=false,
        ymin = 0.45,
        ymax=1.05,
        ytick= {0.5,0.6,0.7,0.8,0.9,1.0},
        yticklabels={0.5,0.6,0.7,0.8,0.9,1.0},
        ytick align = outside,
        ytick pos = left,
        max space between ticks=1000pt,
        try min ticks=7,
        %
        % xmin=0,
        % xmax=1,
        % xtick = {0.0,0.2,0.4,0.6,0.8,1.0},
        xtick align = outside,
        xtick pos = bottom,
        scaled ticks = false,
        tick label style={/pgf/number format/.cd, fixed, precision=3}
        %
        % grid=both,
        % grid style={line width=.1pt, draw=gray!30},
    ]  
    \ifthenelse{\equal{#4}{1}}{
        \addlegendimage{line legend, blue0, line width = 1}
        \addlegendentry{vanilla}  
        \addlegendimage{line legend, orange1, line width = 1}
        \addlegendentry{constrained}  
    }{}
    \foreach \column in {0,...,24}    
    {
        \foreach \model/\c in {
            vanilla/blue0,
            constrained/orange1
        }
        {
            \edef\temp{
                \noexpand\addplot[
                color=\c,
                line width = .25,
                opacity = .3,
                no marks,
                ] table [x={epsilons}, y = \column, col sep=comma] {figs/adv_examples/\model/#1.csv};
            }
            \temp
        }
    }
    \addplot[
        color=blue0,
        line width = .25,
        dashed
        ] table [x={epsilons}, y = {median}, col sep=comma] {figs/adv_examples/vanilla/#1.csv};
    \addplot[
        color=orange1,
        line width = .25,
        dashed
        ] table [x={epsilons}, y = {median}, col sep=comma] {figs/adv_examples/constrained/#1.csv};
\end{axis}
\end{scope}
}
\begin{tikzpicture}
    \def \xsep{6.8cm}
    \def \ysep{3.5cm}
    \foreach \attack/\x/\y\b\c in {
        FGSM/0/0/1/1,
        FGM/1/0/0/1,
        L2PGD/0/1/0/0,
        LinfPGD/1/1/0/0,
        L2AdditiveUniformNoiseAttack/0/2/0/0,
        L2AdditiveGaussianNoiseAttack/1/2/0/0,
        GaussianBlurAttack/0/3/0/0,
        L2ContrastReductionAttack/1/3/0/0,
        L2DeepFoolAttack/0.5/4/0/0
        }
    {
        \plotattack{\attack}{{\x*\xsep}}{{-\y*\ysep}}{\b}{\c}
    }
\end{tikzpicture}

